Learning Personalized Decision Support Policies

Individual human decision-makers may benefit from different forms of support to improve decision outcomes, but when each form of support will yield better outcomes? In this work, we posit that personalizing access to decision support tools can be an effective mechanism for instantiating the appropriate use of AI assistance. Specifically, we propose the general problem of learning a decision support policy that, for a given input, chooses which form of support to provide to decision-makers for whom we initially have no prior information. We develop $\texttt{Modiste}$, an interactive tool to learn personalized decision support policies. $\texttt{Modiste}$ leverages stochastic contextual bandit techniques to personalize a decision support policy for each decision-maker and supports extensions to the multi-objective setting to account for auxiliary objectives like the cost of support. We find that personalized policies outperform offline policies, and, in the cost-aware setting, reduce the incurred cost with minimal degradation to performance. Our experiments include various realistic forms of support (e.g., expert consensus and predictions from a large language model) on vision and language tasks. Our human subject experiments validate our computational experiments, demonstrating that personalization can yield benefits in practice for real users, who interact with $\texttt{Modiste}$.

==> TMLR/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> problem_formulation.tex <==
\section{Problem Formulation}

In this section, we provide a formal description of a human decision-making process under various forms of decision support. 
We propose a multi-objective optimization problem to capture trade-offs between the cost of support and the decision outcome for a given form of support. 
We then cast the multi-objective problem into a single-objective and discuss how to evaluate the resultant decision support policy subject to a desired performance threshold.

\subsection{Problem Setting}\label{sec:problem}
We consider a human decision-making process with different forms of decision support. In particular, we focus on a multi-class classification problem with observation/feature space $\gX \subseteq \mathbb{R}^p$ and outcome/label space $\gY = \bss{K}$. 
We concentrate on a stochastic setting where the data $(x,y) \in \gX \times \gY$ are drawn iid from a fixed, unknown data generating distribution $\gP$, an assumption that reflects typical decision-making settings. 
In addition, we consider an action set $\gA$ corresponding to the forms of support available. 
Given an observation $x \in \gX$, the human attempts to predict the corresponding label $y \in \gY$ using the support prescribed by an action $a \in \gA$, i.e., the human makes the prediction using an unknown function $h: \gX \times \gA \to \gY$. 
\textit{Our problem formulation and algorithms to solve the formulation are agnostic to the specific forms of support}; we provide multiple instantiations in later human subject experiments.
The cost of using different support is given by $c: \gA \to [0,1]$. The quality of the final prediction made by the human is measured by a loss function $\ell: \gY \times \gY \to [0,1]$ w.r.t. the true label. We consider a 0-1 loss function, where $\ell(y, y') = 1$ for $y \ne y'$ and $\ell(y, y') = 0$ for $y = y'$.  





\paragraph{Decision-Making Protocol.} 
We aim to learn a policy $\pi: \gX \to \Delta(\gA)$ that picks the appropriate form of support to assist a new
decision-maker. Let $\Pi$ denote the class of all stochastic decision support policies. Let $\gA = \bcc{\textsc{A}_1, \ldots, \textsc{A}_k}$, and $\pi(x)_{\textsc{A}_i}$ denote $\mathbb{P}[\textsc{A}_i \sim \pi(x)]$ for each $\textsc{A}_i \in \gA$. 
When $\textsc{A}_i \sim \pi(x)$, the human decision-maker makes the prediction $\widetilde{y}$ based on the observation $x$ and support prescribed by $\textsc{A}_i$, i.e., the final prediction $\widetilde{y}$ is given by $\widetilde{y} = h(x, \textsc{A}_i)$. The human decision-making process with different forms of support is described below. For $t = 1,2,\dots,T$:
\begin{enumerate}[leftmargin=*,labelindent=4pt]
\itemsep0em
\item A data point $(x_t, y_t) \in \gX \times \gY$ is drawn iid from $\gP$.
\item A form of support $a_t \in \gA$ is selected using a decision support policy $\pi_t: \gX \to \Delta(\gA)$.
\item The human decision-maker makes the final prediction $\widetilde{y}_t = h(x_t, a_t)$ based on $x_t$ and $a_t$.
\item The human decision-maker incurs a loss $\ell(y_t, \widetilde{y}_t) = 1$ if $y_t \ne \widetilde{y}_t$ and $\ell(y_t, \widetilde{y}_t) = 0$ otherwise.
\end{enumerate}




\looseness-1A static decision support policy, where the policy does not change throughout the interaction with the decision-maker, could be deployed. This approach reflects many prior user studies, per ~\citet{lai2021towards}; for example, decision-makers may \emph{always} be presented with the predictions of an ML model. Additionally, it is possible to update a policy $\pi_t$ iteratively at each time step based on the most recent interaction with the decision-maker, i.e., using $\{(x_t, y_t, a_t, \widetilde{y}_t)\}$. We propose a method to make such an update online in Section~\ref{sec:algo}.




\subsection{Learning Objectives}\label{sec:opt_form}

\looseness-1At each time step $t$, we evaluate the current policy $\pi_t$ based on two objectives: (i) the loss of the decision-maker's prediction under the form of support selected by the policy $\pi_t$, and (ii) the cost associated with that form of support. We formalize these objectives below.


\looseness-1For any policy $\pi$, the expected loss incurred by the decision-maker under policy $\pi$ is given by:
\begin{equation}\label{eq:risk}
    \begin{split}
        r_h(\pi) &~=~ \mathbb{E}_{(x,y) \sim \gP} \big[\mathbb{E}_{\textsc{A}_i \sim \pi(x)}[\ell (y, h(x, \textsc{A}_i))]\big]
        ~=~ \mathbb{E}_x \bigg[\sum_{i=1}^k{\pi(x)_{\textsc{A}_i} \cdot \mathbb{E}_{y|x}[\ell (y, h(x, \textsc{A}_i))]}\bigg] .
    \end{split}
\end{equation}
Further, the expected cost of the policy $\pi$ is given by:
\begin{equation}\label{eq:cost}
    c(\pi) = \mathbb{E}_x \bigg[\sum_{i=1}^k{\pi(x)_{\textsc{A}_i} \cdot c(\textsc{A}_i)}\bigg].
\end{equation}


Given these two objectives, we consider the following multi-objective optimization (MOO):
\begin{equation}
\label{eq:moop}
\min_\pi ~ \gR_h(\pi) ~=~ [r_h(\pi) , c(\pi)]^\top .
\end{equation}
In subsequent evaluations, irrespective of the method used to learn a decision support policy, we evaluate the quality of a policy at a given time $\pi_t$ by considering its expected loss $r_h(\pi_t)$, and expected cost $c(\pi_t)$.  
We use expected performance to measure generalization across inputs, rather than instantaneous performance on a single data point $(x_t, y_t)$.










\subsection{Reframing the Objective}


We first reformulate this MOO problem into a single-objective optimization (SOO) problem:
\begin{equation}
\label{eq:soop}
\pi^*_\lambda ~=~ \argmin_{\pi \in \Pi} \lambda \cdot r_h(\pi) + (1 - \lambda) \cdot c(\pi) ,
\end{equation}
where $\lambda \in [0, 1]$. 
It can be shown that the solutions of the SOO problem can fully characterize the Pareto front of the MOO problem, i.e., any Pareto optimal policy of the MOO problem is a solution to the SOO problem for some choice of $\lambda \in [0,1]$~\citep{mas1995microeconomic,branke2008multiobjective}. The formal statements are provided in Appendix~\ref{app:pareto}. 
For any given $\lambda \in [0,1]$, our goal is to develop an online learning algorithm to find the solution $\pi^*_\lambda$ to the SOO problem in Eq.~\ref{eq:soop}. 
We observe that we can rewrite the SOO problem as follows (see Appendix~\ref{app:reframing}):
\begin{equation}
\label{eq:soop-solution}    
\pi^*_\lambda(x) ~=~ \argmin_{\textsc{A}_i \in \mathcal{A}} \lambda \cdot \br{p_{\textsc{A}_i}(x; h)} + (1 - \lambda) \cdot c(\textsc{A}_i) ,
\end{equation}
where $r_{\textsc{A}_i}(x; h) = \mathbb{E}_{y|x}[\ell (y, h(x, \textsc{A}_i))]$ is the human prediction error for input $x$ and support $\textsc{A}_i$. 
This simplified form of $\pi^*_\lambda$ enables us to propose an efficient strategy to learn the policy online by estimating $r_{\textsc{A}_i}(x; h)$ value via interaction with the decision-maker $h$.
It is nontrivial to identify the appropriate modeling assumptions for $h$ under all forms of support~\citep{kim2008human}; thus, for the purposes of learning which form of support to provide, we focus on learning $r_{\textsc{A}_i}(x;h)$ for a given $h$.






\subsection{Evaluating Policies in Practice}

In practice, we want to learn a policy that achieves a certain level of performance at a minimal cost.
That is, given a tolerance threshold $\epsilon \in [0,1]$ for the expected loss, our goal is to learn a decision support policy $\pi$ that achieves minimum expected cost while maintaining the expected loss that is within $\epsilon$ of the optimal loss $r_h^\text{opt}$: 
\begin{equation}
\label{eq:coop}
\pi^\epsilon ~=~ \argmin_{\pi \in \Pi} ~ c(\pi) \quad \text{such that}  \quad r_h(\pi) \leq r_h^\text{opt} + \epsilon , 
\end{equation}
where $r_h^\text{opt} = \min_\pi r_h(\pi)$. However, it is unclear what the corresponding choice of $\lambda$ is, if any, for a given $\epsilon$ and $h$. 
We observe that there exists a $\lambda(\epsilon) \in [0,1]$ such that $\pi^*_{\lambda(\epsilon)} = \pi^\epsilon$ where $\pi^\epsilon \in \Pi_\text{opt} = \{\pi^*_\lambda: \lambda \in [0,1] \}$ and $\Pi_h^\text{opt}$ is the complete set of Pareto optimal policies for a given human $h$. 
Thus, we propose a hyper-parameter tuning strategy to find a $\lambda$ that leads to a policy with an expected loss of no more than $\epsilon$ above $r_h^\text{opt}$.












\section{Methods} 
\label{sec:algo}



When faced with a new decision-maker, a lack of prior information can make it challenging to learn a personalized decision support policy. Obtaining an extensive offline dataset of human decision-making for an unseen decision-maker \textit{with every form of support} may be difficult in practice. While we may have access to data from other decision-makers in the population, relying solely on population-level data may not suffice for a new decision-maker, who may have individual differences in how they make decisions or rely on support.
In contrast to the discussion in Section~\ref{sec:related}, we propose a framework (Figure~\ref{fig:dspoverview}) for learning decision support policies \emph{online}.\footnote{If we had additional information via offline datasets or prior knowledge on the new human decision-maker, we can likely incorporate that information into selecting $\lambda(\epsilon)$ or obtaining more accurate estimates of $\widehat{r}_{\textsc{A}_i}(x; h)$ efficiently; however, considering such additional information is out of scope for this work.} 


\begin{figure*}[tb]
\centering
  \includegraphics[scale=0.35]{figures/figure1_v5.png}
  \caption{We illustrate the process of learning a decision support policy $\pi_t$ online to improve a decision-maker's performance at a minimal added cost. For every decision, our policy selects a form of support $\pi_t(x_t)$ from a set $\mathcal{A}$ (e.g., $a_1 = \text{No support}$, $a_2 = \text{Displaying predictions}$, $a_3 = \text{Consulting experts}$) to present 
  for an input $x_t$. The policy is updated using $\ell(\Tilde{y}_t, y_t)$, the loss incurred after observing a decision $\Tilde{y}_t$. Our online formulation (1) provides policies for new decision-makers for whom no offline data has been collected and (2) personalizes a decision support policy to individual needs. 
  }
  \label{fig:dspoverview}
\end{figure*}


First, in Section~\ref{sec:thread_alone}, we present an online learning algorithm, \texttt{THREAD}, to learn a decision support policy $\pi^*_\lambda$ for any given $\lambda \in [0,1]$ using Eq~\ref{eq:soop-solution}. 
To identify a parameter to deploy for a new decision-maker, we discuss a hyper-parameter tuning strategy that uses population-level data from either interaction data of other decision-makers or estimates of their $r_{\textsc{A}_i}(x; h)$ in Section~\ref{sec:thread_hyper}.
Exploring sample-efficient strategies that jointly identify suitable $\lambda(\epsilon)$ and the corresponding policy $\pi^\epsilon$ is worthy of further investigation. 






\subsection{\texttt{THREAD}}
\label{sec:thread_alone}
The human decision-making process with different forms of support, described in Section~\ref{sec:problem}, can be modeled as a contextual bandit problem, where the forms of support are the arms and $\gX$ is the context space. Based on this insight, we present \texttt{THREAD}, outlined in Algorithm~\ref{alg:DSP}. \texttt{THREAD} is an algorithm 
for learning the policy $\pi^*_\lambda$ online to solve Eq~\ref{eq:soop-solution} for a given $\lambda \in [0,1]$.
We propose Steps 1 and 2 of the algorithm in a general way to work with any online learning method.



\begin{algorithm}
\caption{\texttt{THREAD}}\label{alg:rpu}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} trade-off parameter $\lambda$; human decision-maker $h$; cost function $c: \gA \to [0,1]$
    \STATE \textbf{Initialization:} data buffer $\gD_0 = \{\}$; human prediction error values $\{ \widehat{r}_{\textsc{A}_i, 0} (x; h) = 0.5 : x \in \gX, \textsc{A}_i \in \gA \}$; initial policy $\pi_1$
    \FOR{$t = 1, 2, \dots, T$}
    \STATE data point $(x_t, y_t) \in \gX \times \gY$ is drawn iid from $\gP$
    \STATE support $a_t \in \gA$ is selected using policy $\pi_t$
    \STATE human makes the prediction $\widetilde{y}_t$ based on $x_t$ and $a_t$
    \STATE human incurs the loss $\ell(y_t, \widetilde{y}_t)$
    \STATE update the buffer $\gD_t \gets \gD_{t-1} \cup \bcc{(x_t, a_t, \ell(y_t, \widetilde{y}_t))}$
    \STATE update the decision support policy: \vspace{-2mm}
    \begin{align*}
    \widehat{r}_{\textsc{A}_i, t} (x; h) ~\gets~& \gU_{r}(\widehat{r}_{\textsc{A}_i, t-1} (x; h), \gD_t) \tag{Step 1} \\
    \pi_{t+1}(x) ~\gets~& \gU_{\pi}(\widehat{r}_{\textsc{A}_i, t}, c,  \lambda) \tag{Step 2}
    \end{align*}
    \ENDFOR{}
    \STATE \textbf{Output:} policy $\pi_\lambda^\text{alg} \gets \pi_{T+1}$
  \end{algorithmic}
  \label{alg:DSP}
\end{algorithm}


\paragraph{Policy Update Step 1.} 
In Eq.~\ref{eq:soop-solution}, the costs of each support are given and fixed. The main unknown is the decision-maker's prediction error under different forms of support. We discuss two approaches to estimate the human prediction error $r_{\textsc{A}_i} (x; h)$ for all $x \in \gX$ and $\textsc{A}_i \in \gA$.

\looseness-1First, we use LinUCB~\citep{li2010contextual} to approximate expected loss $r_{\textsc{A}_i} (x; h)$ by a linear function, i.e., $r_{\textsc{A}_i}(x; h) \approx \widehat{r}_{\textsc{A}_i}(x; h) := \ipp{\theta_{\textsc{A}_i}}{x}$. We learn the parameters $\bcc{\theta_{\textsc{A}_i}: \textsc{A}_i \in \gA}$ using LinUCB with the instantaneous reward function $R(x, y, \textsc{A}_i; h) := \ell(y, h(x, \textsc{A}_i))$. We then normalize the values of $\widehat{r}_{\textsc{A}_i}(x; h)$ to lie in the range $[0,1]$. 


Second, we use an intuitive $K$-nearest neighbor (KNN) approach, which is a simplified variant of KNN-UCB~\citep{guan2018nonparametric}, to approximate the error values $r_{\textsc{A}_i}(x; h)$. Specifically, we maintain an evolving data buffer $\gD_t$, where we accumulate the history of interactions with the decision-maker. For any new observation $x$, we can estimate $\widehat{r}_{\textsc{A}_i}(x; h)$ values by finding its $K$-nearest neighbors in $\gD_t$ and computing the average error of these neighbors.





\paragraph{Policy Update Step 2.}
\looseness-1As mentioned above, it is crucial to have accurate estimates of the human prediction error values (see Eq~\ref{eq:soop-solution}). To achieve this, one could use a pure exploratory policy $\pi_{t+1}$ in Step 2 of Algorithm~\ref{alg:DSP}, where $\pi_{t+1}(x)_{\textsc{A}_i} = 1/\abs{\gA}$ for all $\textsc{A}_i \in \gA$. However, this approach would require a large number of interactions $T$ to achieve accurate error estimates. In practical settings, where interactions are limited, as in our human subject experiments, $T$ tends to be relatively small, making this approach less feasible.

When trying to learn the policy $\pi^*_\lambda$ for a given $\lambda$, one can improve sample efficiency by guiding exploration with the policy $\pi_{t+1}(x) = \argmin_{\textsc{A}_i \in \mathcal{A}} \lambda \cdot \widehat{r}_{\textsc{A}_i,t}(x; h) + (1 - \lambda) \cdot c(\textsc{A}_i)$ in Step 2 of Algorithm~\ref{alg:DSP}. Additionally, depending on the specific implementation, additional exploration terms can be used for better performance. In Appendix~\ref{app:algo-context}, we present specific implementations of Algorithm~\ref{alg:DSP} using LinUCB and online KNN. 


\subsection{Hyper-parameter selection for \texttt{THREAD}} 
\label{sec:thread_hyper}



While we introduce multiple algorithm-specific parameters in Section~\ref{sec:thread_alone} (e.g., $\alpha$ for LinUCB and $K$, $W$, and $\gamma$ for KNN), the hyper-parameter of primary interest is $\lambda(\epsilon)$.\footnote{From here on, we drop the explicit dependence on $\epsilon$ for more concise notation.}
When learning a decision support policy online for a new decision-maker $h$, we need to identify a suitable $\lambda$ that achieves an expected loss within $\epsilon$ of $r_h^\text{opt}$. 
However, it is difficult to test multiple $\lambda$ values simultaneously for the new decision-maker without potentially repeating queries of the same input: we only have a finite number of interactions with the decision-maker before issues of cognitive load arise per Section~\ref{sec:user_study}.
We now describe a strategy to select 
$\lambda$ using population-level data. While the decision-makers in the population may differ from the unseen decision-maker, we prefer this principled starting point to a random selection of $\lambda$.

\paragraph{Constructing human simulators.}
For each of the $m$ decision-makers in our population-level data, we construct a simulator by calculating $r_{\textsc{A}_i}(x; h_j)$ for all $\textsc{A}_i$, $x \in \mathcal{X}$, and $j \in [m]$. 
Each $r_{\textsc{A}_i}(x; h_j)$ is \emph{agnostic} to the instantiation of the form of support and does not explicitly model how the decision-maker $j$ leverages $\textsc{A}_i$. 
To capture human competencies across $\mathcal{X}$, we assume that the input space is divided into regions where $r_{\textsc{A}_i}(x; h)$ is roughly the same across that region for a given form of support $\textsc{A}_i$. 
These regions may be defined by class labels or by covariates of the task. 
For example, we write $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$ to denote that, under observing support $\textsc{A}_1$, the decision-maker incurs a risk of $0.7$ on one region, of $0.1$ on a second, and $0.7$ on the third.
We let $\{h_{\text{sim-}1},\ldots,h_{\text{sim-}m}\}$ denote the set of simulated decision-makers.


\paragraph{Selecting a trade-off parameter for deployment.} We want to select a trade-off parameter to deploy \texttt{THREAD} with for an unseen human $h_\text{real}$. As a result, we apply \texttt{THREAD} (with the same cost structure $c(\textsc{A}_i)$ as that of the real decision-maker) on each simulated decision-maker $h_{\text{sim-}j}$ across a range of $\lambda$ values to obtain a set of candidate policies. 
In our experiments, we evaluate a range of $\lambda \in [0,1]$ values in increments of $0.05$. 
From this set of candidate policies and their respective $\lambda$ values, we decide which $\lambda$ to deploy on $h_\text{real}$.
We consider three selection strategies: 
\begin{enumerate}
    \item[A.] \textbf{Most likely $\lambda$.} For each simulator, we identify the set of $\{\lambda_{\text{sim-}j}\}$, which yield policies that meet $r_{h_{\text{sim-}j}}^\text{opt} + \epsilon$. We then take the $\lambda$ that occurs the \emph{most often} across simulators. If no policy meets the threshold for $h_{\text{sim-}j}$ , we select the policy closest to $r_{h_{\text{sim-}j}}^\text{opt}$, which can be computed given $r_{\textsc{A}_i}$ for all $x$ for each simulated decision-maker. 

    \item[B.] \textbf{Most likely $\lambda$ with lowest cost.}  For each simulator, we identify the set of $\{\lambda_{\text{sim-}j}\}$, which yield policies that meet $r_{h_{\text{sim-}j}}^\text{opt} + \epsilon$, and select the $\lambda$ whose policy has the least expected cost. Then, we identify the most common value across simulators. While the set of values here is a subset of the selection strategy A, a cost-aware selection strategy may identify a parameter that leads to a lower cost for new decision-makers.

     \item[C.] \textbf{Conservative $\lambda$.} For each simulator, we identify $\lambda_{\text{sim-}j}$ which is the minimum parameter that meets $r_{h_{\text{sim-}j}}^\text{opt} + \epsilon$. We then take $\max_j \lambda_{\text{sim-}j}$ over all simulated decision-makers.  In the absence of suitable population-level information, this strategy is similar to picking a conservative value of $\lambda$ that prioritizes performance.
\end{enumerate}

\noindent We note further considerations for evaluating our proposed strategy in Appendix~\ref{appdx:performance}.


==> table.tex <==

\begin{table*}[t!]
\centering
\footnotesize
% \scriptsize
\caption{
We report the expected loss $L_h(\pi)$ and the expected cost $c(\pi)$---for both metrics, lower is better---averaged across the last 10 steps of 100 total time steps along with their standard deviations (across 5 runs) for various human simulators instantiated using synthetic and real data.
% For Synthetic-$2A$ and CIFAR-$2A$, we learn policies for synthetic humans, whose risks are denoted in Table~\ref{tab:results}.
For CIFAR-$3A$ and MMLU-$2A$, we learn policies for three individuals from the observed population per Appendix~\ref{appdx:popconstruct}: the decision-maker with the lowest risk on their own (i.e., without support), the decision-maker with the lowest Best Risk, and the decision-maker with the highest Best Risk. We report the values of $\lambda$ selected for each person in Table~\ref{tab:lambda_values}.
We \textbf{bold} the algorithm that achieves the lowest cost within $\epsilon$ risk of the Best Risk for each human simulator, and find that our algorithm outperforms baselines on various simulated humans. 
\vccomment{condense caption}
% For \texttt{THREAD}, we select the best policy over a sweep of $\lambda$ values that minimizes Eq.~\ref{eq:coop} under $\epsilon = 0.05$.
}
% Synthetic Population
% \resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
% \hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
% $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
% $r_{\textsc{A}_2} = [0.1, 0.1, 0.1]$\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
% $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
% $r_{\textsc{A}_2} = [0.1, 0.7, 0.1]$ 
% \end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
% $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
% $r_{\textsc{A}_2} = [0.7, 0.7, 0.1]$\\ \end{tabular}} \\ 
% \cline{3-8} 
%   & \small{Algorithm}        & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                             & $c(\pi)$                            \\ \hline
% \multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Synthetic-$2A$\\ 
% % (CIFAR separable)
% \end{tabular}}} 
% % & Human alone ($\pi^*_{\lambda=0}$)    
% & \small{$\textsc{A}_1$ Only }    
% & \multicolumn{1}{c|}{$0.51 \pm 0.05$}    &     $0.0$       & 
%  \multicolumn{1}{c|}{$0.50 \pm 0.06$}    &     $0.0$       & 
% \multicolumn{1}{c|}{$0.50 \pm 0.06$}    &     $0.0 $                                   \\ \cline{2-8}  
% \multicolumn{1}{c|}{}                                                                                       
% % & Human+model   
% & \small{$\textsc{A}_2$ Only}
% & \multicolumn{1}{c|}{$0.10 \pm 0.03$}    &     $0.5$       & 
%  \multicolumn{1}{c|}{$0.30 \pm 0.05$}    &     $0.5 $       & 
% \multicolumn{1}{c|}{$0.50 \pm 0.04$}    &     $0.5 $                                   \\ \cline{2-8}  
% \multicolumn{1}{c|}{}                                                                                       
% & \small{Population}       
% & \multicolumn{1}{c|}{$0.37 \pm 0.04$}    &     $0.13 \pm 0.03$       
% & \multicolumn{1}{c|}{$0.34 \pm 0.05$}    &     $0.13 \pm 0.02$      
% & \multicolumn{1}{c|}{$0.49 \pm 0.06$}    &     $0.12 \pm 0.03$                                   \\ \cline{2-8} 
% \multicolumn{1}{c|}{}   

% % & \small{Human Pop }       
% % & \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$       & 
% %  \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$      & 
% % \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$                                   \\ \cline{2-8}  
% % \multicolumn{1}{c|}{}    
% & \small{\texttt{THREAD}-LinUCB}   
% & \multicolumn{1}{c|}{$\mathbf{0.15 \pm 0.05}$}    &     $\mathbf{0.31 \pm 0.03}$       & 
%  \multicolumn{1}{c|}{$0.12 \pm 0.04$}    &     $0.32 \pm 0.03$       & 
% \multicolumn{1}{c|}{$0.34 \pm 0.11$}    &     $0.28 \pm 0.07$                                   \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                                                                       
% & \small{\texttt{THREAD}-KNN}     & \multicolumn{1}{c|}{$0.11 \pm 0.04$}    &     $0.36 \pm 0.03$       & 
%  \multicolumn{1}{c|}{$\mathbf{0.13 \pm 0.04}$}    &     $\mathbf{0.30 \pm 0.03}$       & 
% \multicolumn{1}{c|}{$\mathbf{0.33 \pm 0.06}$}    &     $\mathbf{0.21 \pm 0.03}$                                   \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                                                                       & 
% \small{Best Risk } 
% & \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
%  \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
% \multicolumn{1}{c|}{$0.3$}    &     $0.17$                                                                
% \\ \bottomrule
% \end{tabular}}
% % \ \\
% % \ \\
% % \ \\
% \resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
% \hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
% $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
% $r_{\textsc{A}_2} = [0.1, 0.1, 0.1]$\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
% $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
% $r_{\textsc{A}_2} = [0.1, 0.7, 0.1]$ 
% \end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
% $r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
% $r_{\textsc{A}_2} = [0.7, 0.7, 0.1]$\\ \end{tabular}} \\ 
% \cline{3-8} 
%   & \small{Algorithm}        & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                             & $c(\pi)$                            \\ \hline
% \multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR--$2A$\\ \end{tabular}}} & \small{$\textsc{A}_1$ Only}      & \multicolumn{1}{c|}{$0.50 \pm 0.05$}    &     $0.0$       & 
% \multicolumn{1}{c|}{$0.50 \pm 0.05$}    &     $0.0$       & 
% \multicolumn{1}{c|}{$0.47 \pm 0.05$}    &     $0.0$                                         \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                                                                       & \small{$\textsc{A}_2$ Only}         
% & \multicolumn{1}{c|}{$0.1 \pm 0.03$}    &     $0.5$       & 
% \multicolumn{1}{c|}{$0.31 \pm 0.04$}    &     $0.5$       & 
% \multicolumn{1}{c|}{$0.49 \pm 0.05$}    &     $0.5$                                       
% \\ \cline{2-8} \multicolumn{1}{c|}{}                                                                                      
% & \small{Population}      
% & \multicolumn{1}{c|}{$0.46 \pm 0.07$}    &     $0.03 \pm 0.04$       & 
% \multicolumn{1}{c|}{$0.43 \pm 0.06$}    &     $0.07 \pm 0.03$       & 
% \multicolumn{1}{c|}{$0.50 \pm 0.06$}    &     $0.03 \pm 0.02$                                       
% \\ \cline{2-8} \multicolumn{1}{c|}{}    
% % & \small{Human Pop }       
% % & \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$       & 
% %  \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$      & 
% % \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$                                  
% % \cline{2-8}  
% % \multicolumn{1}{c|}{}    
% & 
% \small{\texttt{THREAD}-LinUCB}  & \multicolumn{1}{c|}{$\mathbf{0.15 \pm 0.04}$}    &     $\mathbf{0.31 \pm 0.02}$       & 
% \multicolumn{1}{c|}{$\mathbf{0.14 \pm 0.05}$}    &     $\mathbf{0.32 \pm 0.02}$       & 
% \multicolumn{1}{c|}{$0.34 \pm 0.07$}    &     $0.25 \pm 0.07$                                      
% \\ \cline{2-8} \multicolumn{1}{c|}{}                                          & \small{\texttt{THREAD}-KNN}    & \multicolumn{1}{c|}{$0.14 \pm 0.04$}    &     $0.33 \pm 0.06$       & 
% \multicolumn{1}{c|}{$\mathbf{0.14 \pm 0.04}$}    &     $\mathbf{0.32 \pm 0.03}$       & 
% \multicolumn{1}{c|}{$\mathbf{0.33 \pm 0.05}$}    &     $\mathbf{0.18 \pm 0.03}$                                     
% \\ \cline{2-8} \multicolumn{1}{c|}{}                                                                                  & \small{Best Risk }
% & \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
% \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
% \multicolumn{1}{c|}{$0.3$}    &     $0.17$                                    \\ \bottomrule 
% \end{tabular}}
% \ \\
% \ \\
% \ \\
% Human Population
\resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
\hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
Best alone
% $r_{\textsc{H-Only}} = [0.0, 0.8, 0.7, 0.3, 0.2]$\\ 
% $r_{\textsc{H-Model}} = [0.0, 0.4, 0.2, 0.6, 0.6]$\\
% $r_{\textsc{H-Consensus}} = [0.0, 1.0, 0.4, 0.0,0.0]$
\end{tabular}} & 
\multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
Lowest best risk
% $r_{\textsc{H-Only}} = [0.0, 0.3, 0.7, 0.8, 0.9]$\\ 
% $r_{\textsc{H-Model}} = [0.0, 0.0, 0.0, 1.0, 1.0]$\\
% $r_{\textsc{H-Consensus}} = [0.1, 0.6, 0.7, 0.1, 0.1]$
\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
Highest best risk
% $r_{\textsc{H-Only}} = [0.0, 0.7, 0.9, 0.7, 0.4]$\\ 
% $r_{\textsc{H-Model}} = [0.0, 0.7, 0.3, 0.7, 0.8]$\\
% $r_{\textsc{H-Consensus}} = [0.0, 0.6, 0.7, 0.3, 0.4]$
\end{tabular}} \\ \cline{3-8} 
  & \small{Algorithm}        & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                             & $c(\pi)$                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR--$3A$\end{tabular}}} & \small{\textsc{H-Only}   }
 & \multicolumn{1}{c|}{$0.42 \pm  0.05$}    &     $0.0$       & 
 \multicolumn{1}{c|}{$0.52 \pm  0.06$}    &     $0.0$       & 
\multicolumn{1}{c|}{$0.54 \pm 0.05$}    &     $0.0$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & \small{\textsc{H-Model} Only}   
&  \multicolumn{1}{c|}{$0.33 \pm  0.05$}    &     $0.5$       & 
 \multicolumn{1}{c|}{$0.41 \pm 0.05$}    &     $0.5$       & 
\multicolumn{1}{c|}{$0.50 \pm 0.05$}    &     $0.5$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & \small{\textsc{H-Consensus} Only}       
& \multicolumn{1}{c|}{$0.27 \pm 0.03$}    &     $0.5$       & 
 \multicolumn{1}{c|}{$0.41 \pm 0.06$}    &     $0.5$       & 
\multicolumn{1}{c|}{$0.40 \pm 0.04$}    &     $0.5$                                   \\ \cline{2-8}  
\multicolumn{1}{c|}{}                                                                                       & \small{Population}       
& \multicolumn{1}{c|}{$0.42 \pm 0.05$}    &     $0.01 \pm 0.01$       & 
 \multicolumn{1}{c|}{$0.54 \pm 0.03$}    &     $0.01 \pm 0.01$      & 
\multicolumn{1}{c|}{$0.53 \pm 0.05$}    &     $0.01 \pm 0.01$                                   \\ \cline{2-8}  
\multicolumn{1}{c|}{}                                                                                       & \small{\texttt{THREAD}-LinUCB }
& \multicolumn{1}{c|}{$0.23 \pm 0.06$}    &     $0.34 \pm 0.08$       & 
 \multicolumn{1}{c|}{$0.21 \pm 0.08$}    &     $0.38 \pm 0.08$       & 
\multicolumn{1}{c|}{$0.43 \pm 0.09$}    &     $0.32 \pm 0.08$                                   
\\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       
& \small{\texttt{THREAD}-KNN }    
& \multicolumn{1}{c|}{$0.21 \pm 0.05$}    &     $0.32 \pm 0.07$       & 
 \multicolumn{1}{c|}{$\mathbf{0.11 \pm 0.03}$}    &     $\mathbf{0.39 \pm 0.03}$       & 
\multicolumn{1}{c|}{$\mathbf{0.37 \pm 0.05}$}    &     $\mathbf{0.28 \pm 0.05}$                                  
\\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                      & 
\small{Best Risk   }
& \multicolumn{1}{c|}{$0.12$}    &     $0.4$       & 
 \multicolumn{1}{c|}{$0.06$}    &     $0.4$       & 
\multicolumn{1}{c|}{$0.32$}    &     $0.3$                                     \\ \bottomrule 
\end{tabular}}
% \ \\
% \ \\
% \ \\
\resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
\hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
Best alone
% $r_{\textsc{H-Only}} = [0.3, 0.1, 0.5, 0.3]$\\ 
% $r_{\textsc{H-LLM}} = [0.5, 0.1, 0.0, 0.1]$
\end{tabular}} & 
\multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
Lowest best risk
% $r_{\textsc{H-Only}} = [0.3, 0.9, 0.3, 0.9]$\\ 
% $r_{\textsc{H-LLM}} = [0.0, 0.1, 0.0, 0.3]$
\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
Highest best risk
% $r_{\textsc{H-Only}} = [0.8, 0.6, 0.8, 0.6]$\\ 
% $r_{\textsc{H-LLM}} = [0.6, 0.3, 0.7, 0.1]$
\end{tabular}} \\ \cline{3-8} 
  & \small{Algorithm}        & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                             & $c(\pi)$                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}MMLU--$2A$\end{tabular}}} & \small{\textsc{H-Only}   }
 & \multicolumn{1}{c|}{$0.30 \pm  0.03$}    &     $0.0$       & 
 \multicolumn{1}{c|}{$0.54 \pm  0.05$}    &     $0.0$       & 
\multicolumn{1}{c|}{$0.68 \pm 0.03$}    &     $0.0$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & \small{\textsc{H-LLM} Only}   
&  \multicolumn{1}{c|}{$0.21 \pm 0.03$}    &     $0.1$       & 
 \multicolumn{1}{c|}{$0.09 \pm 0.02$}    &     $0.1$       & 
\multicolumn{1}{c|}{$0.42 \pm 0.06$}    &     $0.1$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & \small{Population}       
& \multicolumn{1}{c|}{$0.13 \pm 0.03$}    &     $0.05 \pm 0.01$       & 
 \multicolumn{1}{c|}{$0.35 \pm 0.07$}    &     $0.05 \pm 0.01$      & 
\multicolumn{1}{c|}{$0.53 \pm 0.05$}    &     $0.05 \pm 0.01$                                   \\ \cline{2-8}  
\multicolumn{1}{c|}{}                                                                                       & \small{\texttt{THREAD}-LinUCB }
& \multicolumn{1}{c|}{$0.15 \pm 0.05$}    &     $0.04 \pm 0.01$       & 
 \multicolumn{1}{c|}{$0.20 \pm 0.10$}    &     $0.05 \pm 0.02$       & 
\multicolumn{1}{c|}{$0.51 \pm 0.06$}    &     $0.06 \pm 0.01$                                   
\\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       
& \small{\texttt{THREAD}-KNN }    
& \multicolumn{1}{c|}{$\mathbf{0.17 \pm 0.03}$}    &     $\mathbf{0.03 \pm 0.01}$       & 
 \multicolumn{1}{c|}{$\mathbf{0.12 \pm 0.03}$}    &     $\mathbf{0.08 \pm 0.01}$       & 
\multicolumn{1}{c|}{$\mathbf{0.46 \pm 0.05}$}    &     $\mathbf{0.06 \pm 0.01}$                                  
\\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                      & 
\small{Best Risk   }
& \multicolumn{1}{c|}{$0.13$}    &     $0.08$       & 
 \multicolumn{1}{c|}{$0.09$}    &     $0.1$       & 
\multicolumn{1}{c|}{$0.42$}    &     $0.1$                                     \\ \bottomrule 
\end{tabular}}
\label{tab:results}
\end{table*}

==> table_cost.tex <==
\begin{table*}[t!]
\centering
\footnotesize
% \scriptsize
\caption{
In the cost-aware setting for MMLU-$2A$, we compare the expected loss $L_h(\pi)$ and the expected cost $c(\pi)$ (lower is better) averaged across the last 10 steps of 100 total time steps of 5 separate runs.
We select two individuals who have a ``varying'' profile 
% (corresponding to decision-makers with the first and second lowest risk without support)
and two individuals who have a ``strictly better'' profile.
% (corresponding decision-makers with the lowest and highest $L_h^\text{opt}$)}.
We follow the described workflow to find a suitable $\lambda$, reported for each person in Table~\ref{tab:lambda_values}.
We \textbf{bold} the algorithm that achieves the lowest cost within $\epsilon=0.05$ risk of each individual $h$'s $L_h^\text{opt}$. 
}
\resizebox{\textwidth}{!}{\begin{tabular}{ccccccccc}\toprule
                   & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
Varying: $L_h^\text{opt} = 0.13$\\
$r_{\textsc{H-Only}} = [0.3, 0.1, 0.5, 0.3]$\\ 
$r_{\textsc{H-LLM}} = [0.5, 0.1, 0.0, 0.1]$ \\ \midrule
\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
% Highest best risk\\
Varying: $L_h^\text{opt} = 0.10$\\
$r_{\textsc{H-Only}} = [0.1, 0.3, 0.6, 0.6]$\\ 
$r_{\textsc{H-LLM}} = [0.4, 0.0, 0.3, 0.0]$ \\ \midrule
\end{tabular}} 
& 
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
Strictly Better: $L_h^\text{opt} = 0.43$\\
$r_{\textsc{H-Only}} = [0.8, 0.6, 0.8, 0.6]$\\ 
$r_{\textsc{H-LLM}} = [0.6, 0.3, 0.7, 0.1]$ \\ \midrule
\end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
Strictly Better: $L_h^\text{opt} = 0.09$\\
$r_{\textsc{H-Only}} = [0.3, 0.9, 0.3, 0.9]$\\ 
$r_{\textsc{H-LLM}} = [0.0, 0.1, 0.0, 0.3]$ \\ \midrule
\end{tabular}} 

\\
   \small{Algorithm}        & \multicolumn{1}{c}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c}{$L_h(\pi)$}                             & $c(\pi)$     & \multicolumn{1}{c}{$L_h(\pi)$}                             & $c(\pi)$                        \\ \midrule
 \small{\textsc{H-Only}  }
 & \multicolumn{1}{c}{$0.30 \pm  0.03$}    &     $0.0$       & 
 \multicolumn{1}{c}{$0.41 \pm  0.04$}    &     $0.0$       & 
\multicolumn{1}{c}{$0.68 \pm 0.03$}    &     $0.0$ &
\multicolumn{1}{c}{$0.54 \pm 0.05$}    &     $0.0$ \\ 
\small{\textsc{H-LLM}}   
&  \multicolumn{1}{c}{$0.21 \pm 0.03$}    &     $0.1$       & 
 \multicolumn{1}{c}{$0.16 \pm 0.04$}    &     $0.1$       & 
\multicolumn{1}{c}{$0.42 \pm 0.06$}    &     $0.1$    
 & 
\multicolumn{1}{c}{$0.09 \pm 0.02$}    &     $0.1$  \\ 
\small{Population}       
& \multicolumn{1}{c}{$0.13 \pm 0.03$}    &     $0.05 \pm 0.01$       & 
 \multicolumn{1}{c}{$0.16 \pm 0.04$}    &     $0.05 \pm 0.01$      & 
\multicolumn{1}{c}{$0.53 \pm 0.05$}    &     $0.05 \pm 0.01$                                   
 & 
\multicolumn{1}{c}{$0.35 \pm 0.07$}    &     $0.05 \pm 0.01$  \\  
\small{\texttt{Modiste}-LinUCB }
& \multicolumn{1}{c}{$0.15 \pm 0.05$}    &     $0.04 \pm 0.01$       & 
 \multicolumn{1}{c}{$\mathbf{0.15 \pm 0.04}$}    &    $\mathbf{0.06 \pm 0.01}$         & 
\multicolumn{1}{c}{$0.51 \pm 0.06$}    &     $0.06 \pm 0.01$                                   
 & 
\multicolumn{1}{c}{$0.20 \pm 0.10$}    &     $0.06 \pm 0.01$  \\ 
\small{\texttt{Modiste}-KNN }    
& \multicolumn{1}{c}{$\mathbf{0.17 \pm 0.03}$}    &     $\mathbf{0.03 \pm 0.01}$       & 
 \multicolumn{1}{c}{$0.15 \pm 0.04$}    &        $0.07 \pm 0.01$       & 
\multicolumn{1}{c}{$\mathbf{0.46 \pm 0.05}$}    &     $\mathbf{0.05 \pm 0.02}$                                 & 
\multicolumn{1}{c}{$\mathbf{0.12 \pm 0.03}$}    &     $\mathbf{0.08 \pm 0.01}$   
\\ 
\bottomrule 
\end{tabular}}
\label{tab:results}
\vspace{-.25cm}
\end{table*}

==> table_hse.tex <==
\begin{table*}[tb]
    \centering
    \caption{
    \vccomment{get rid of cost, rewrite caption, need to explain observations}
    We report expected loss $L_h(\pi)$ (lower is better) in the last 10 trials by Prolific participants for each Algorithm and \textbf{bold} the variant with the lowest $L_h(\pi)$. }
    % \texttt{Modiste} learns effective, low-cost policies: for CIFAR, \texttt{Modiste} outperforms all baselines; for MMLU, we find that \texttt{Modiste} learns a policy with roughly the same performance as the best offline policy but at \textit{half} the cost.}
    \begin{minipage}{0.48\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\begin{tabular}{ccc}
        \toprule

Algorithm                                  & $L_h(\pi)$      & $c(\pi)$         \\ \midrule
\textsc{H-Only}                                 & $0.68 \pm 0.13$ & $0$             \\ 
\textsc{H-Model}                                 & $0.50 \pm 0.11$ & $0.5$           \\ 
\textsc{H-Consensus}                                & $0.32 \pm 0.07$ & $0.5$           \\ 
Population                                 & $0.66 \pm 0.08$ & $0$           \\ 
\texttt{Modiste}-LinUCB  & $0.22 \pm 0.15$ & $0.38 \pm 0.06$ \\ 
\texttt{Modiste}-KNN      & $\mathbf{0.1 \pm 0.06}$ & $\mathbf{0.44 \pm 0.07}$ \\ 

% \texttt{Modiste}-LinUCB ($\lambda = 0.85$) & $0.5 \pm 0.15$ & $0.14 \pm 0.07$ \\ 

% \texttt{Modiste}-KNN ($\lambda = 0.75$)     & $0.14 \pm 0.23$ & $0.39 \pm 0.06$ \\ 
\bottomrule
\end{tabular}}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\begin{tabular}{ccc} \toprule

Algorithm                                   & $L_h(\pi)$      & $c(\pi)$        \\ \midrule
\textsc{H-Only}                                 & $0.51 \pm 0.14$ & $0$             \\ 
\textsc{H-LLM}                                 & $\mathbf{0.22 \pm 0.14}$ & $\mathbf{0.1}$           \\ 
Population                                 & $0.33 \pm 0.19$ & $0.06 \pm 0.01$           \\ 

\texttt{Modiste}-LinUCB  & $0.25 \pm 0.11$ & $0.05 \pm 0.02$ \\ 

\texttt{Modiste}-KNN      & $0.3 \pm 0.05$ & $0.07\pm 0.02$ \\ 

% \texttt{Modiste}-LinUCB ($\lambda = 0.95$) & $0.35 \pm 0.14$ & $0.04 \pm 0.01$ \\ 
% \texttt{Modiste}-KNN ($\lambda = 0.75$)     & $0.3 \pm 0.11$ & $0.07 \pm 0.02$ \\ 
\bottomrule
% \texttt{Modiste} (KNN, $\lambda = 1.0$, Expert)     & $0.15 \pm 0.11$ & $0.04 \pm 0.03$ \\ 

\end{tabular}} 
    \end{minipage}
        \label{table:hse-results}
\end{table*}

==> table_lambda.tex <==
\begin{table*}[htb]
\scriptsize
\centering
\caption{The best value of $\lambda$ that is selected from doing a sweep over $\lambda \in [0,1]$ that corresponds to the human simulators in Table~\ref{tab:results}. The column ordering is the same as the main paper.}

\begin{tabular}{cc|c|c|c|c}
\hline
 & Algorithm     & \begin{tabular}[c]{@{}c@{}}Best Alone\end{tabular} & \begin{tabular}[c]{@{}c@{}}Second Best Alone\end{tabular} & \begin{tabular}[c]{@{}c@{}}Highest Best Risk\end{tabular} & \begin{tabular}[c]{@{}c@{}}Lowest Best Risk\end{tabular} \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{CIFAR-$3A$}}
% & THREAD-LinUCB &  $0.85$    &    $0.8$        &       $0.9$         \\ \cline{2-5} 
% \multicolumn{1}{c|}{}                          
% & THREAD-KNN    &  $1.0$    &         $0.9$              &          $0.9$              \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{MMLU-$2A$}} 
& \texttt{Modiste}-LinUCB &   $0.7$   &  $0.65$ &   $1.0$     &         $0.95$         \\ \cline{2-6} 
\multicolumn{1}{c|}{}                          
& \texttt{Modiste}-KNN    &   $0.25$   &  $0.55$ &    $0.35$                &          $0.6$           \\ \hline
\end{tabular}
\label{tab:lambda_values}
\end{table*}


==> table_old.tex <==

\begin{table*}[htb]
\centering
\footnotesize
% \scriptsize
\caption{We instantiate simulated \textbf{synthetic} humans, each specified by the human's loss on each form of support \textsc{H-Only} (Human only) and \textsc{H-Model} (Human+Model), for MMLU-$2A$.
We report the expected loss $r_h(\pi)$ and the expected cost $c(\pi)$---for both metrics, lower is better---averaged across the last 10 steps of 100 total time steps along with their standard deviations (across 5 runs). 
We bold the algorithm that achieves the lowest cost within $\epsilon$ of the Best Risk for each human simulation and find that our algorithm outperforms baselines on various simulated humans. 
For each form of support, we specify risk $r$ over each of the 4 topics for MMLU-$2A$. We fix the cost structure: $c(\textsc{H-Only}) = 0.0$ and  $c(\textsc{H-Model}) = 0.1$.
The selected $\lambda$ values used for \texttt{Modiste} are in Table~\ref{tab:lambda_values}.
For \texttt{Modiste}, we select the best policy over a sweep of $\lambda$ values that minimizes our objective under $\epsilon = 0.05$. We also indicate the values of $\lambda$ chosen beneath the results table. 
}

\resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
\hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.1, 0.1, 0.1]$\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.1, 0.7, 0.1]$ 
\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.7, 0.7, 0.1]$\\ \end{tabular}} \\ 
\cline{3-8} 
  & \small{Algorithm}        & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                             & $c(\pi)$                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Synthetic-$2A$\\ 
% (CIFAR separable)
\end{tabular}}} 
% & Human alone ($\pi^*_{\lambda=0}$)    
& \small{$\textsc{A}_1$ Only }    
& \multicolumn{1}{c|}{$0.51 \pm 0.05$}    &     $0.0$       & 
 \multicolumn{1}{c|}{$0.50 \pm 0.06$}    &     $0.0$       & 
\multicolumn{1}{c|}{$0.50 \pm 0.06$}    &     $0.0 $                                   \\ \cline{2-8}  
\multicolumn{1}{c|}{}                                                                                       
% & Human+model   
& \small{$\textsc{A}_2$ Only}
& \multicolumn{1}{c|}{$0.10 \pm 0.03$}    &     $0.5$       & 
 \multicolumn{1}{c|}{$0.30 \pm 0.05$}    &     $0.5 $       & 
\multicolumn{1}{c|}{$0.50 \pm 0.04$}    &     $0.5 $                                   \\ \cline{2-8}  
\multicolumn{1}{c|}{}                                                                                       
& \small{Population}       
& \multicolumn{1}{c|}{$0.37 \pm 0.04$}    &     $0.13 \pm 0.03$       
& \multicolumn{1}{c|}{$0.34 \pm 0.05$}    &     $0.13 \pm 0.02$      
& \multicolumn{1}{c|}{$0.49 \pm 0.06$}    &     $0.12 \pm 0.03$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}   

% & \small{Human Pop }       
% & \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$       & 
%  \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$      & 
% \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$                                   \\ \cline{2-8}  
% \multicolumn{1}{c|}{}    
& \small{\texttt{Modiste}-LinUCB}   
& \multicolumn{1}{c|}{$\mathbf{0.15 \pm 0.05}$}    &     $\mathbf{0.31 \pm 0.03}$       & 
 \multicolumn{1}{c|}{$0.12 \pm 0.04$}    &     $0.32 \pm 0.03$       & 
\multicolumn{1}{c|}{$0.34 \pm 0.11$}    &     $0.28 \pm 0.07$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       
& \small{\texttt{Modiste}-KNN}     & \multicolumn{1}{c|}{$0.11 \pm 0.04$}    &     $0.36 \pm 0.03$       & 
 \multicolumn{1}{c|}{$\mathbf{0.13 \pm 0.04}$}    &     $\mathbf{0.30 \pm 0.03}$       & 
\multicolumn{1}{c|}{$\mathbf{0.33 \pm 0.06}$}    &     $\mathbf{0.21 \pm 0.03}$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & 
\small{Best Risk } 
& \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
 \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
\multicolumn{1}{c|}{$0.3$}    &     $0.17$                                                                
\\ \bottomrule
\end{tabular}}
% \ \\
% \ \\
% \ \\
\resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
\hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.1, 0.1, 0.1]$\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.1, 0.7, 0.1]$ 
\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.7, 0.7, 0.1]$\\ \end{tabular}} \\ 
\cline{3-8} 
  & \small{Algorithm}        & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$L_h(\pi)$}                             & $c(\pi)$                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR--$2A$\\ \end{tabular}}} & \small{$\textsc{A}_1$ Only}      & \multicolumn{1}{c|}{$0.50 \pm 0.05$}    &     $0.0$       & 
\multicolumn{1}{c|}{$0.50 \pm 0.05$}    &     $0.0$       & 
\multicolumn{1}{c|}{$0.47 \pm 0.05$}    &     $0.0$                                         \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & \small{$\textsc{A}_2$ Only}         
& \multicolumn{1}{c|}{$0.1 \pm 0.03$}    &     $0.5$       & 
\multicolumn{1}{c|}{$0.31 \pm 0.04$}    &     $0.5$       & 
\multicolumn{1}{c|}{$0.49 \pm 0.05$}    &     $0.5$                                       
\\ \cline{2-8} \multicolumn{1}{c|}{}                                                                                      
& \small{Population}      
& \multicolumn{1}{c|}{$0.46 \pm 0.07$}    &     $0.03 \pm 0.04$       & 
\multicolumn{1}{c|}{$0.43 \pm 0.06$}    &     $0.07 \pm 0.03$       & 
\multicolumn{1}{c|}{$0.50 \pm 0.06$}    &     $0.03 \pm 0.02$                                       
\\ \cline{2-8} \multicolumn{1}{c|}{}    
% & \small{Human Pop }       
% & \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$       & 
%  \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$      & 
% \multicolumn{1}{c|}{$0.00 \pm 0.00$}    &     $0.00 \pm 0.00$                                  
% \cline{2-8}  
% \multicolumn{1}{c|}{}    
& 
\small{\texttt{Modiste}-LinUCB}  & \multicolumn{1}{c|}{$\mathbf{0.15 \pm 0.04}$}    &     $\mathbf{0.31 \pm 0.02}$       & 
\multicolumn{1}{c|}{$\mathbf{0.14 \pm 0.05}$}    &     $\mathbf{0.32 \pm 0.02}$       & 
\multicolumn{1}{c|}{$0.34 \pm 0.07$}    &     $0.25 \pm 0.07$                                      
\\ \cline{2-8} \multicolumn{1}{c|}{}                                          & \small{\texttt{Modiste}-KNN}    & \multicolumn{1}{c|}{$0.14 \pm 0.04$}    &     $0.33 \pm 0.06$       & 
\multicolumn{1}{c|}{$\mathbf{0.14 \pm 0.04}$}    &     $\mathbf{0.32 \pm 0.03}$       & 
\multicolumn{1}{c|}{$\mathbf{0.33 \pm 0.05}$}    &     $\mathbf{0.18 \pm 0.03}$                                     
\\ \cline{2-8} \multicolumn{1}{c|}{}                                                                                  & \small{Best Risk }
& \multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
\multicolumn{1}{c|}{$0.1$}    &     $0.33$       & 
\multicolumn{1}{c|}{$0.3$}    &     $0.17$                                    \\ \bottomrule 
\end{tabular}}
\resizebox{\textwidth}{!}{\begin{tabular}{cc|cc|cc|cc}
\hline  &                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.8, 0.8, 0.1, 0.1]$\\ 
$r_{\textsc{A}_2} = [0.2, 0.1, 0.1, 0.2]$\end{tabular}} & 
\multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.2, 0.8, 0.1, 0.1]$\\ 
$r_{\textsc{A}_2} = [0.8, 0.1, 0.1, 0.2]$\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.2, 0.5, 0.5, 0.8]$\\ 
$r_{\textsc{A}_2} = [0.8, 0.1, 0.1, 0.8]$\end{tabular}} \\ \cline{3-8} 
  & \small{Algorithm}        & \multicolumn{1}{c|}{$r_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$r_h(\pi)$}                         & $c(\pi)$                         & \multicolumn{1}{c|}{$r_h(\pi)$}                             & $c(\pi)$                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}MMLU-$2A$\end{tabular}}} & \small{\textsc{H-Only}  ($\pi^*_{\lambda=0}$)  }
 & \multicolumn{1}{c|}{$0.45 \pm  0.04$}    &     $0.0$       & 
 \multicolumn{1}{c|}{$0.33 \pm  0.06$}    &     $0.0$       & 
\multicolumn{1}{c|}{$0.51 \pm 0.04$}    &     $0.0$                                   \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       & \small{\textsc{H-Model}}   
&  \multicolumn{1}{c|}{$0.14 \pm 0.02$}    &     $0.1$       & 
 \multicolumn{1}{c|}{$0.30 \pm 0.05$}    &     $0.1$       & 
\multicolumn{1}{c|}{$0.45 \pm 0.04$}    &     $0.1$                                   \\ \cline{2-8} 

\multicolumn{1}{c|}{}                                                                                       & \small{Human Pop }       
& \multicolumn{1}{c|}{$0.45 \pm 0.07$}    &     $0.05 \pm 0.01$       & 
 \multicolumn{1}{c|}{$0.22 \pm 0.08$}    &     $0.06 \pm 0.01$      & 
\multicolumn{1}{c|}{$0.41 \pm 0.04$}    &     $0.05 \pm 0.01$                                   \\ \cline{2-8}  
\multicolumn{1}{c|}{}                                                                                       & \small{\texttt{Modiste}-LinUCB }
& \multicolumn{1}{c|}{$0.15 \pm 0.04$}    &     $0.05 \pm 0.06$       & 
 \multicolumn{1}{c|}{$0.19 \pm 0.07$}    &     $0.05 \pm 0.02$       & 
\multicolumn{1}{c|}{$0.39 \pm 0.08$}    &     $0.06 \pm 0.01$                                   
\\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                       
& \small{\texttt{Modiste}-KNN }    
& \multicolumn{1}{c|}{$\mathbf{0.14 \pm 0.06}$}    &     $\mathbf{0.04 \pm 0.01}$       & 
 \multicolumn{1}{c|}{$\mathbf{0.13 \pm 0.04}$}    &     $\mathbf{0.03 \pm 0.04}$       & 
\multicolumn{1}{c|}{$\mathbf{0.33 \pm 0.05}$}    &     $\mathbf{0.05 \pm 0.01}$                                  
\\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                      & 
\small{Best Risk ($\pi^*_{\lambda=1}$)  }
& \multicolumn{1}{c|}{$0.13$}    &     $0.05$       & 
 \multicolumn{1}{c|}{$0.13$}    &     $0.03$       & 
\multicolumn{1}{c|}{$0.3$}    &     $0.05$                                     \\ \bottomrule 
\end{tabular}}
\ \\
\ \\
\ \\
Selected $\lambda$ Values
\resizebox{\textwidth}{!}{\begin{tabular}{cc|c|c|c}
\hline
 & Algorithm     & \begin{tabular}[c]{@{}c@{}}$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.1, 0.1, 0.1]$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.1, 0.7, 0.1]$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r_{\textsc{A}_1} = [0.7, 0.1, 0.7]$\\ 
$r_{\textsc{A}_2} = [0.7, 0.7, 0.1]$\end{tabular} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Synthetic-$2A$}}
& \texttt{Modiste}-LinUCB &  $0.4$    &    $0.6$        &       $0.6$         \\ \cline{2-5} 
\multicolumn{1}{c|}{}                          
& \texttt{Modiste}-KNN    &  $0.9$    &         $0.6$              &          $0.6$              \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{CIFAR-$2A$}} 
& \texttt{Modiste}-LinUCB &   $0.4$   &     $0.9$      &      $0.5$         \\ \cline{2-5} 
\multicolumn{1}{c|}{}                          
& \texttt{Modiste}-KNN    &   $0.7$   &      $0.9$                &          $0.6$           \\ \hline
\end{tabular}}
\ \\
\ \\
\ \\
\resizebox{\textwidth}{!}{\begin{tabular}{cc|c|c|c}
\hline
 & Algorithm     & \begin{tabular}[c]{@{}c@{}}$r_{\textsc{A}_1} = [0.8, 0.8, 0.1, 0.1]$\\ 
$r_{\textsc{A}_2} = [0.2, 0.1, 0.1, 0.2]$\end{tabular} & \begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.2, 0.8, 0.1, 0.1]$\\ 
$r_{\textsc{A}_2} = [0.8, 0.1, 0.1, 0.2]$\end{tabular}&
\begin{tabular}[c]{@{}c@{}}
$r_{\textsc{A}_1} = [0.2, 0.5, 0.5, 0.8]$\\ 
$r_{\textsc{A}_2} = [0.8, 0.1, 0.1, 0.8]$\end{tabular}\\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{MMLU-$2A$}}
& \texttt{Modiste}-LinUCB    &   $1.0$   &      $0.9$        &          $1.0$       \\ \cline{2-5} 
\multicolumn{1}{c|}{}                          
& \texttt{Modiste}-KNN    &   $0.3$   &      $0.2$                &          $0.3$         \\ \hline
\end{tabular}}
\label{tab:results_synth}
\end{table*}
